Coupling OpenFOAM(R) with BoSSS, a discontinuous Galerkin solver written in C#

In this article, we present the foam-dg project, which provides a bridge between OpenFOAM(R) and the high-order DG (discontinuous Galerkin) framework BoSSS. Thanks to the flexibility of the coupling approach, mixed calculations where some parts of the equation system are solved in OpenFOAM(R) and others are solved in BoSSS are easily possible. This is showcased using the convective Cahn-Hilliard equation, where the Cahn-Hilliard part is solved in BoSSS and the Navier-Stokes part is solved in OpenFOAM(R). The obtained results appear reasonable, though the main focus of this paper is to present and document the foam-dg project rather than on quantitative results.

==> parts/author-contributions.tex <==
The OpenFOAM Journal requires the contributions of all authors to be explicitly stated
As noted below, please see \href{http://img.mdpi.org/data/contributor-role-instruction.pdf}{CRediT taxonomy} for the term explanation.
Replace the example authors initials (F.A., S.A) below as appropriate

Please turn to http://img.mdpi.org/data/contributor-role-instruction.pdf (CRediT taxonomy) for the term explanation.

\authorcontributions{
Conceptualisation, J.S.;
methodology, J.S.;
software, J.S;
validation, J.S. and P.M.;
formal analysis, J.S. and P.M.;
investigation, J.S.;
resources, P.M.;
data curation, P.M.;
writing---original draft preparation, J.S.;
writing---review and editing, J.S. and P.M.;
visualisation, J.S.;
supervision, P.M.;
project administration, P.M.;
funding acquisition, P.M.
All authors have read and agreed to the published version of the manuscript.
}

